Metabolic graphs, LIFE method and the modeling of drug action on Mycobacterium tuberculosis

This paper serves as a framework for designing advanced models for drug action on metabolism. Drug treatment may affect metabolism by either enhancing or inhibiting metabolic reactions comprising a metabolic network. We introduce the concept of \textit{metabolic graphs}, a generalization of hypergraphs having specialized features common to metabolic networks. Linear-in-flux-expression (briefly LIFE) is a methodology for analyzing metabolic networks and simulating virtual patients. We extend LIFE dynamics to be compatible with metabolic graphs, including the more complex interactions of enhancer and inhibitor molecules that affect biochemical reactions. We discuss results considering network structure required for existence and uniqueness of equilibria on metabolic graphs and show simulations of drug action on \textit{Mycobacterium tuberculosis} (briefly MTB)

==> HOC.tex <==
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\U{{\mathcal U}}
\def\xd{\dot x}
\def\Ppi{\textsl{\bf{P}} }
\def\Cci{\textsl{\bf{C}}}
\def\nat{{I\!\!N}}

\noindent
If $\Sigma$ is a hybrid system, then a \textit{Lagrangian} for $\Sigma$ is a family $L=\{ L_q\}_{q\in Q}$, $L_q:\real^n\times U_q\to\real$ and
an endpoint cost function is a family of real-valued functions
$\varphi=\{\varphi_{q,q'}\}_{(q,q')\in Q\times Q}$. 
Given $L$ and $\varphi$, a  {\it cost functional}  $C$ is defined setting
\[
C(\textbf{X})  =  \sum_{j=1}^\nu
\int_{t_{j-1}}^{t_j}L_{q_j}(x_j(t),u_j(t))\,dt
+\varphi_{q_1,q_\nu}(x_1(t_0),x_{\nu}(t_\nu)),
\]
where $\textbf{X}$ is a trajectory for $\Sigma$.
Given an initial condition $(q_0,x_0)$, 
an hybrid optimal control  problem
${\cal P}(q_0,x_0)$
is defined as the minimization of 
$C$ over all hybrid trajectories starting from $(q_0,x_0)$.
As in classical control, the value function is defined as:
\[
V(q_0,x_0)=\inf_{\textbf{X}\ s.t.\ \textbf {X}(0)=(q_0,x_0)} C(\textbf{X}).
\]
For classical control systems it is known that, under suitable conditions, the value function $V$ is the unique (viscosity) solution to a Partial Differential Equation
called Hamilton-Jacobi-Bellmann, see \cite{BCD97} and (\ref{eq:HJB}) below.
A method to find optimal controls consists in the following steps (see
\cite{BP04,MR2996162,MR3408272} for more detail):\\
1. Find candidate optimal trajectories $Y(q_0,x_0)$
for initial data $(q_0,x_0)$ on an open region.\\
2. Compute the corresponding candidate value function
$W(q_0,x_0)=C(Y(q_0,x_0))$.\\
3. Verify that $W$ coincides with $V$, so that
all trajectories $Y(q_0,x_0)$ are optimal.\\
The collection $\{Y(q_0,x_0)\}$ is called synthesis and can be constructed, under suitable conditions, using the well-known Pontryagin Maximum Principle (briefly PMP, a fist order necessary condition for optimality, see \cite{bressan2007introduction}) and geometric control techniques. 
In the rest of the Section we illustrate how this program works and how to extend it to the hybrid setting.
The PMP has been already extended to the hybrid case by various authors \cite{garavello2005hybrid,SC07,S99}.\\

\noindent
{\bf Sufficient conditions: Value function approach.}
Sufficient conditions are known for a candidate value function $W$ to coincide with the value
function $V$ (\cite{MR2996162}):
\begin{theorem}\label{tm8.5}
%Let $\Omega\subseteq\R^{n+1}$ be an open subset and 
Let $W:\overline{\Omega}\mapsto\real$, $\Omega$ open, 
be a continuous function such that:\\
i) $W \ge V$ and
at every point $(t,x) \in \partial \Omega$, one has
$W(t,x)= M \doteq \sup_{(s,y)\in\Omega} W(s,y)$;\\
ii) there exist finitely many manifolds $\M_1,\cdots,\M_N
\subset  \Omega$ with dimension $\le n$, 
such that $W$ is continuously
differentiable on the set $\Omega\backslash \cup \M_i$
and satisfies the Hamilton-Jacobi equation
\begin{equation}\label{eq:HJB}
W_s(s,y) + \min_{u\in U(s,y)} \{ W_y(s,y)\cdot f(s,y,u) \} =0.
\end{equation}
Then $W$ coincides with the value function $V$ on the domain $Q$.
\end{theorem}
To extend to hybrid system, our main idea is the following. First we will construct
a candidate value function on the starting location $q_0$ (for MTB corresponding to 
the metabolic state in normal conditions) on a region containing the switching set ${\cal S}$. 
Then we will extend to the other locations via boundary conditions along the switching set.\\


\noindent
{\bf Sufficient condition: Optimal synthesis.}
An alternative method is to provide conditions directly
on the synthesis assuming that all trajectories satisfy the PMP
and the synthesis is generated by a sufficiently smooth feedback $u(x)$
on a stratification. In simple words, a stratification is a partition
with manifolds of different dimension called strata 
(plus some regularity condition), the feedback is smooth on each stratum
and its trajectories travel over a finite number of strata. 
For a precise description, we need to introduce some notation.\\
%A {\em synthesis} on an open set $\Omega$ is a collection of trajectories $\Gamma=\{\gamma_{x}:x\in\Omega, \gamma_{x}{\rm \ steers\ }x{\rm\ to\ }S\}$, and $\Gamma$ is {\em optimal} if every $\gamma_{x}$ is.  We consider the case in which $\Gamma$ is generated by a feedback which is piecewise smooth on a stratification.
A set $P\subset\real^n$ is said a {\it curvilinear open
polytope} of dimension $p$ if $\phi(P'\setminus\partial P')=P$
with $P'\subset \real^{p}$ polytope and $\phi:\real^p\to\real^n$,
injective with Jacobian of maximal rank at every point.\\
Let $\Omega$ be an open set, then
$\Gamma$ is a {\it Boltyanskii--Brunovsky regular synthesis} 
on $\Omega$, briefly BB synthesis, if the following holds.
There exists a 6--tuple $\Xi=(\Ppi,\Ppi_1,\Ppi_2,\Pi,\Sigma,u)$
such that\\
(BB1) $\Ppi$ is a  finite collection of curvilinear polytopes, $\Omega$ is disjoint union of elements of $\Ppi$.\\
%If $P_j\not=P_k\in\Ppi$ and $P_k\cap \overline{P_j}\not=\emptyset$ then $P_k\subset \partial P_j$ and $\dim(P_k)<\dim(P_j)$.\\
% $\{0\}\in \Ppi$ and the elements of $\Ppi$ are called ``cells''.\\
(BB2) $\Ppi$ is the disjoint union of
$\Ppi_1$ (`type I strata'') and $\Ppi_2$ (``type II strata''),\\
(BB3) $u$ is defined on type I strata,
%:\{x:\exists P_1\in \Ppi_1, x\in P_1\} \rightarrow U$ and 
$\Pi:\Ppi_1\rightarrow\Ppi$ assigns new strata for curves on
type I strata and the multifunction
$\Sigma:\Ppi_2\rightarrow\Ppi_1$ for curves
on type II strata. Moreover:\\
%is a multifunction, with non empty values, such that the following properties are satisfied:\\
i) The function $u$ is of class $C^1$ on each stratum.\\
ii) For each $x$ on a type I cell $P_1$, let $t_x$ be the maximal time of existence for the maximal solution $\xi_x$ of the feedback $u$ on $P_1$.
Then  $\xi_x(t_x-):=\lim_{t\uparrow t_x}\xi_x(t)\in\Pi(P_1)$.\\
iii) For each $x$ on a type II cell $P_2$ and each $P\in\Sigma(P_2)$,
there exists a unique trajectory $\xi_x^P$ of $u$ from $x$ exiting $P_2$ 
then running on $P$.\\
iv) On every type I cell $P_1$, $x\to t_x$ and and $(t,x)\to\xi_x(t)$
are continuously differentiable functions.
%$(t,x)\to u_x(t):= u(\xi_x(t))$ are continuously differentiable
%maps on the set
%$E(P):=\{(t,x):x\in P_1\,,\,t\in[0,t_x]\}.$
%in the sense that they can be prolonged to maps of class $\Cci^1$ on
%some open subset of $\real\times P_1$ containing $E(P_1)$.
If $P_2$ is of type II, the same holds for every $t_x^P$, $\xi_x^P$,
$u_x^P$, with $P\in\Sigma(P_2)$.\\
v) For every $x\in \Omega$, the synthesis trajectory
$\gamma_x:[0,T_x]\to\real^n$, $\gamma_x\in\Gamma$, is obtained by
piecing together the trajectories on strata. and changes stratum a finite number of times.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=10cm]{BB.pdf}
%\caption{Example of BB synthesis.}\label{fig:BBsyn}
%\end{center}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{remark} Notice that condition (BB1) essentially means that the collection of open polyhedra form a ``triangulation" of the set $\Omega$.
%, see Figure \ref{fig:BBsyn}. 
%In the same figure we represent the two type of cells to illustrate properties (BB2) and (BB3). 
%The cell $P_1$ is of type I and dimension equal
%to 2, then there are trajectories running on it, corresponding to
%the feedback $u$, which end on the cell $\Pi(P_1)$. On the
%contrary, the cell $P_2$ is of type II and dimension equal to 1,
%hence from every point there start some trajectories entering other
%cells. More precisely, from every point of $P_2$ it starts one
%trajectory entering the 2-dimensional cell $P_3$ and one entering
%the 2-dimensional cell $P_4$, this means
%$\Sigma(P_2)=\{P_3,P_4\}$.
%\end{remark}
For BB synthesis the following holds (\cite{PS00}):
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}{\bf (Sufficiency theorem for BB syntheses.)}\label{c8:th:BB}
Let $\Gamma$ be a BB synthesis formed by trajectories satisfying PMP, then $\Gamma$ is optimal.
\end{theorem}
%
\begin{remark}
BB synthesis may be defined using general manifolds
and Whitney stratified set. For a complete presentation see \cite{PS00}.
\end{remark}
The generalization to hybrid system will be achieved using the Hybrid Maximum Principle
\cite{garavello2005hybrid,SC07,S99} and a feedback which is regular on a stratification on each location. 
Then we will provide "gluing" conditions for feedback trajectories switching locations also using approximation by smooth problems
as in \cite{HT11}.



==> Hybrid.tex <==
\subsection{Biology of Gene Regulatory Network for MTB}
Mycobacterium tuberculosis is known to thrive in environments that would be considered hostile to similar bacteria. A major source of MTB's versatility is its Gene Regulatory Network (briefly GRN), which allows it to abruptly shift its metabolic network in order to survive. This happens when MTB encounters environmental conditions such as hypoxia, nitric oxide stress, or varying nutritional availability \cite{balazsi2008temporal,lee2006flux,peterson2014high}.
Investigations into the GRN of MTB have discovered novel regulatory mechanisms; 454 of these were discovered for gene regulation activated by stressful environments, cholesterol utilization, and dormancy \cite{minch2015dna,peterson2014high,raman2009flux}.
The complexity and sophistication of the GRN must be accounted for in the design of new models. %treatments, and further investigations into the GRN will complement our proposed modeling strategy. 
%To this end, efforts have been made to reconstruct the co-regulated genes under certain culture conditions using high-throughput microarray analysis. This method can uncover when genes are members of many different co-regulated gene groups which is consistent with the underlying biology and elucidates combinatorial regulation by environmental factors as well as the transcription factors that enforce the GRN.

%Our analysis of the GRN data showed the following:\\
%{\tt TODO Summarize the finding}


\subsection{Regulatory flux balance analysis approach}
To design successful treatments for tuberculosis, one needs to  anticipate the metabolic responses to drugs, in particular capturing the GRN reaction and the consequent change in metabolic states of MTB. 
The Flux Balance Analysis approach (briefly FBA) was successfully
applied to many biological networks, see \cite{gianchandani2010application,kauffman2003advances,orth2010flux,palsson2015systems}.
. 
However, when the GRN has a large effect on the system, FBA may provide incorrect predictions, see \cite{covert2001regulation, gianchandani2010application}, thus FBA
was modified into the regulatory Flux Balance Analysis (briefly rFBA, see \cite{covert2001regulation}) which accounts for different metabolic states. rFBA uses boolean operators to allow a switch of metabolic states when a flux or metabolite exceeds a threshold, or a flux vanish possibly from depletion of nutrients.\\ 
To identify the biologically feasible steady states of the system, FBA constructs cones in the flux space guaranteeing positivity of all fluxes
(which are connected via Kirchhoff-type relations at nodes) as in
Fig. \ref{fig:FBA} left. 
The edges of these flux cones correspond to extreme pathways,
which are special paths connecting intakes to excretions and
can be identified via an algorithm from the stoichiometric matrix
see \cite{merrill2019stability,palsson2015systems}.
Non-negative  combinations of extreme pathways generate all feasible flow through the network. 
Such flux cones change when the metabolic state switches
%and it is compared to a similar feasible flux region resulting 
or when a flux is deactivated by the GRN,  see Fig \ref{fig:FBA} right,
thus affecting equilibria and dynamics of the network.

\begin{figure}[!h]
\begin{center}
\input{FBAtikz.tex}
%\includegraphics[scale=0.5]{TB_GRN.PNG}
\caption{\footnotesize Left: biologically feasible cone of positive fluxes,
with edges corresponding to extreme pathways.
Right: modified cone resulting from deactivation of a basis vector.}\label{fig:FBA}
\end{center}
\end{figure}

\subsection{Hybrid systems approach}
A dynamic system comprising a continuous dynamics (as that of metabolites) combined with a discrete one (as that of metabolic states) is often referred to as \emph{hybrid system} and there is a wide literature
for such systems and their optimal control, see for instance \cite{AHLP00,AKNS95,BBDBSV02,BFM00,BBM98,CPW01,garavello2005hybrid,GST09,hedlund1999optimal,
Lygeros1999ControllersFR,piccoli1998hybrid,SC07,S99,TPS98,VDSS98}.
We will use hybrid control systems methods to study the dynamics of MTB metabolic networks under the action of drugs, including the effect of GRN on switching of metabolic states. A first simple representation is given in figure \ref{fig:hybrid}.
\begin{figure}[ht]
\begin{center}
\input{hybrid_system.tex}
%\includegraphics[scale=0.5]{TB_GRN.PNG}
\caption{\footnotesize A hybrid system of two metabolic states.}\label{fig:hybrid}
\end{center}
\end{figure}
Here we assume two metabolic states: $M_1$ and $M_2$
and the network dynamics is given by the corresponding 
stoichiometric matrices $S_1$ and $S_2$.
The switching in metabolic states are triggered by the two
conditions $x\leq D$ and $x\geq C$ (interpreted as vector inequalities,
i.e. for all components of metabolite vector $x$).\\
%rFBA combined with Linear-In-Flux systems will facilitate modeling the response of MTB to treatment.  We propose to combine these methodologies through the control theory of Hybrid systems \cite{piccoli1998hybrid}.  Hybrid systems are those with continuous and discrete variables. In this proposed research, the different metabolic states are discrete, and the metabolites are continuous and we will formulate a hybrid system control problem.
More generally a hybrid control system is comprised of continuous variables $x$ and discrete ones $q$ called \emph{locations}, representing discrete variables such as metabolic states.
Formally a hybrid control system on $\real^n$ is a 4-tuple
\mbox{$\Sigma=(Q,U,f,{\cal S})$} such that:
$Q$ is a finite set;  
$U=\{U_q\}_{q\in Q}$ is a family of control sets;
$f=\{f_{q}\}_{q\in Q}$ is a family of controlled dynamics
$f_q:\real^n\times U_{q}\mapsto \real^n$;
the switching set ${\cal S}$ is a subset of  
$\{(q,x,q',x')\!:\!q,q'\!\!\in\! Q,x,x'\in\real^n\}$.
A hybrid state is a couple $(q,x)$, 
where $q\in Q$ is the location and $x\in\real^n$ is the state.
%The definition of hybrid systems may be more complicated allowing different state spaces, control sets, etc., we refer the reader to\cite{piccoli1998hybrid} for details.
The evolution of the hybrid system is as follows.
Given a hybrid initial state $(q_1,x_0)$, at time $t_0$, 
on some time interval $[t_0,t_1[$ the system evolves solving:
$q(t)\equiv q_1$ and 
$\dot x(t)=f_{q_1}(x(t),u_1(t))$ for some admissible control $u_1$.
If the solution to the previous system can be prolonged on the whole
interval $[t_0,t_1]$, then
we can choose another hybrid state $(q_2,x_1)$, 
such that $(q_1,x(t_1),q_2,x_1)\in{\cal S}$ 
and let the system evolve in location $q_2$ following the corresponding
controlled dynamics and so on.
\begin{remark}
Here we are presenting a special class of hybrid systems. More generally, each location may have different state space and set of admissible controls. Moreover, one can introduce various time and switching constraints, we refer to \cite{garavello2005hybrid,GST09,piccoli1998hybrid,S99} for details.
\end{remark}
We will define an hybrid system generalizing that of Figure \ref{fig:hybrid}
and formulate and solve an optimal control problem corresponding to maximizing the drug inhibition of MTB, following the strategy of next Section.

